Top-quark properties at ATLAS

Properties of the top-quark are presented, with emphasis on the most recent ATLAS measurements of the mass and $t\bar{t}$ spin correlations, obtained with proton-proton collision data collected at the Large Hadron Collider. Normalised differential distributions are used in both cases. For the extraction of the top-quark mass, $t\bar{t}+1$-jet single-lepton events are selected from the 20.2 fb$^{-1}$ 8 TeV dataset, and the unfolded distribution at parton level is compared with theoretical predictions to obtain $m_t^{\text{pole}} = 171.1^{+1.2}_{-1.1}$ GeV in the pole-mass scheme and $m_t(m_t) = 162.9^{+2.4}_{-1.6}$ GeV in the running-mass scheme. For the measurement of spin correlations in $t\bar{t}$ production, dilepton events are selected using 36.1 fb$^{-1}$ 13 TeV data. The azimuthal opening angle between the two leptons is measured inclusively and as a function of the invariant mass of the $t\bar{t}$ system. The observed degree of spin correlation is significantly higher than predicted by the generators used, but agrees well with the prediction of one of the fixed-order calculations.

==> Makefile <==
LATEX    = latex
BIBTEX   = bibtex
DVIPS    = dvips

BASENAME = main

default: testlatex

review:
	latex  ${BASENAME}
	latex  ${BASENAME}

testlatex:
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}
ifeq ($(TERM_PROGRAM),Apple_Terminal)
	open -a Preview ${BASENAME}.pdf
endif

#
# standard Latex targets
#

%.dvi:	%.tex 
	$(LATEX) $<

%.bbl:	%.tex *.bib
	$(LATEX) $*
	$(BIBTEX) $*

%.ps:	%.dvi
	$(DVIPS) $< -o $@

%.pdf:	%.tex
	$(PDFLATEX) $<

.PHONY: clean

clean:
	rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg  \
	      *.inx *.dvi *.toc *.out *~ ~* spellTmp 


